Recent Developments on the HI Gas of Low-Redshift Galaxies Seen by the 21cm Emission Lines

As a major interstellar medium, the atomic neutral hydrogen (HI) plays an important role in the galaxy evolution. It provides the ingredient for star formation, and sensitively traces the internal processes and external perturbations influencing the galaxy. With the beginning of many new radio telescopes and surveys, HI may make a more significant contribution to the understanding of galaxies in the near future. This review discusses the major development of the $21\,\text{cm}$ emission-line HI observations and studies in the past few years, including its scaling relations with other galaxy properties, its kinematics and structures, its role in environmental studies, and its constraints on hydrodynamical simulations. The local-Universe HI scaling relations of stellar-mass--selected samples extend smoothly to $10^9\,\text{M}_\odot$ stellar mass, with a tentative evolution to the redshift of ${\sim}0.1$. The development of measurement techniques enables better estimations of HI non-circular motion, dispersion, and thickness, and new observations revealed extended or extra-planar HI structures, both helpfully constraining the gas accretion, stellar feedback, and star formation processes of galaxy evolution models. HI is very useful for tracing the on-going satellite evolution in dense environments, the studies of which would benefit from ongoing blind HI surveys. Though simulations still cannot fully reproduce HI gas properties, they help to understand the role of possible factors in regulating HI properties. We also discuss possible future progress with new observations at FAST.

==> journals.tex <==
%auto-ignore
\makeatletter
\let\jnl@style=\relax
\def\ref@jnl#1{{\jnl@style#1}}%
\newcommand\aj{\ref@jnl{Astron. J.}}%
% \newcommand\psj{\ref@jnl{Planetary Science Journal}}%
\newcommand\araa{\ref@jnl{Annu. Rev. Astron. Astr.}}%
\renewcommand\apj{\ref@jnl{Astrophys. J.}}%
\newcommand\apjl{\ref@jnl{Astrophys. J. Lett.}}%
\newcommand\apjs{\ref@jnl{Astrophys. J. Suppl. S.}}%
% \renewcommand\ao{\ref@jnl{Applied Optics}}%
\newcommand\apss{\ref@jnl{Astrophys. Space Sci.}}%
\newcommand\aap{\ref@jnl{Astron. Astrophys.}}%
\newcommand\aapr{\ref@jnl{Astron. Astrophys. Rev.}}%
\newcommand\aaps{\ref@jnl{Astron. Astrophys. Sup.}}%
% \newcommand\azh{\ref@jnl{Astronomicheskii Zhurnal}}%
% \newcommand\baas{\ref@jnl{Bulletin of the AAS}}%
\newcommand\icarus{\ref@jnl{Icarus}}%
% \newcommand\jaavso{\ref@jnl{The Journal of the American Association of Variable Star Observers}}%
% \newcommand\jrasc{\ref@jnl{Journal of the RAS of Canada}}%
% \newcommand\memras{\ref@jnl{Memoirs of the RAS}}%
\newcommand\mnras{\ref@jnl{Mon. Not. R. Astron. Soc.}}%
\renewcommand\pra{\ref@jnl{Phys. Rev. A}}%
\renewcommand\prb{\ref@jnl{Phys. Rev. B}}%
\renewcommand\prc{\ref@jnl{Phys. Rev. C}}%
\renewcommand\prd{\ref@jnl{Phys. Rev. D}}%
\renewcommand\pre{\ref@jnl{Phys. Rev. E}}%
\renewcommand\prl{\ref@jnl{Phys. Rev. Lett.}}%
\newcommand\pasp{\ref@jnl{Publ. Astron. Soc. Pac.}}%
\newcommand\pasj{\ref@jnl{Publ. Astron. Soc. Jpn.}}%
% \newcommand\qjras{\ref@jnl{Quarterly Journal of the RAS}}%
% \newcommand\skytel{\ref@jnl{Sky and Telescope}}%
% \newcommand\solphys{\ref@jnl{Solar Physics}}%
% \newcommand\sovast{\ref@jnl{Soviet Astronomy}}%
% \newcommand\ssr{\ref@jnl{Space Science Reviews}}%
% \newcommand\zap{\ref@jnl{Zeitschrift fuer Astrophysik}}%
\renewcommand\nat{\ref@jnl{Nature}}%
% \newcommand\iaucirc{\ref@jnl{IAU Cirulars}}%
\newcommand\aplett{\ref@jnl{Astrophys. Lett.}}%
% \newcommand\apspr{\ref@jnl{Astrophysics Space Physics Research}}%
% \newcommand\bain{\ref@jnl{Bulletin Astronomical Institute of the Netherlands}}%
% \newcommand\fcp{\ref@jnl{Fundamental Cosmic Physics}}%
% \newcommand\gca{\ref@jnl{Geochimica Cosmochimica Acta}}%
% \newcommand\grl{\ref@jnl{Geophysics Research Letters}}%
% \renewcommand\jcp{\ref@jnl{Journal of Chemical Physics}}%
% \newcommand\jgr{\ref@jnl{Journal of Geophysics Research}}%
% \newcommand\jqsrt{\ref@jnl{Journal of Quantitiative Spectroscopy and Radiative Trasfer}}%
% \newcommand\memsai{\ref@jnl{Mem. Societa Astronomica Italiana}}%
% \newcommand\nphysa{\ref@jnl{Nuclear Physics A}}%
% \newcommand\physrep{\ref@jnl{Physics Reports}}%
% \newcommand\physscr{\ref@jnl{Physica Scripta}}%
% \newcommand\planss{\ref@jnl{Planetary Space Science}}%
% \newcommand\procspie{\ref@jnl{Proceedings of the SPIE}}%

% \newcommand\actaa{\ref@jnl{Acta Astronomica}}%
\newcommand\caa{\ref@jnl{Chinese Astron. Astr.}}%
\newcommand\cjaa{\ref@jnl{Chinese J. Astron. Ast.}}%
% \newcommand\jcap{\ref@jnl{Journal of Cosmology and Astroparticle Physics}}%
% \newcommand\na{\ref@jnl{New Astronomy}}%
% \newcommand\nar{\ref@jnl{New Astronomy Review}}%
\newcommand\pasa{\ref@jnl{Publ. Astron. Soc. Aust.}}%
\newcommand\rmxaa{\ref@jnl{Rev. Mex. Astron. Astr.}}%

%% added feb 9, 2016
% \newcommand\maps{\ref@jnl{Meteoritics and Planetary Science}}
% \newcommand\aas{\ref@jnl{American Astronomical Society Meeting Abstracts}}
% \newcommand\dps{\ref@jnl{American Astronomical Society/Division for Planetary Sciences Meeting Abstracts}}



\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
\makeatother


==> symb.tex <==
\makeatletter
\newcommand\ion[2]{\texorpdfstring{\text{#1\,\textsc{\@roman{#2}}}}{#1 \@roman{#2}}}
\makeatother
\newcommand*{\Hi}{\ion{H}{1}\xspace}
\newcommand*{\sbHi}[1][]{\tsb{\Hi\if\relax\detokenize{#1}\relax\else,#1\fi}\xspace}
\newcommand*{\tsb}[1]{\ensuremath{_{\text{#1}}}}



\newcommand{\fHi}{\ensuremath{f\sbHi}\xspace}
\newcommand{\NHi}{\ensuremath{N\sbHi}\xspace}
\newcommand{\SigHi}{\ensuremath{\Sigma\sbHi}\xspace}
\newcommand{\MHi}{\ensuremath{M\sbHi}\xspace}
\newcommand{\MHZ}{\ensuremath{M\tsb{H\textsubscript{2}}}\xspace}
\newcommand{\dMS}{\ensuremath{\inc\text{MS}}\xspace}
\newcommand{\Rmol}{\ensuremath{R\tsb{mol}}\xspace}
\newcommand{\RHi}{\ensuremath{R\sbHi}\xspace}
\newcommand{\NUV}{\text{NUV}\xspace}
\newcommand{\Rqo}{\ensuremath{R_{90}}\xspace}
\newcommand{\Rso}{\ensuremath{R_{50}}\xspace}
\newcommand{\Rzoo}{\ensuremath{R_{200}}\xspace}

\makeatletter
\@ifpackageloaded{unicode-math}{%
  \newcommand{\inc}{\increment}
}{%
  \newcommand{\inc}{\Delta}
}\makeatother
\makeatother


% units
\DeclareSIUnit\yr{yr}
\DeclareSIUnit\Gyr{\giga\yr}
\DeclareSIUnit\Myr{\mega\yr}
\DeclareSIUnit\G{G}
\DeclareSIUnit\uG{\micro\G}
\DeclareSIUnit\pc{pc}
\DeclareSIUnit\Msun{M\ensuremath{_\odot}}
\DeclareSIUnit\kpc{\kilo\pc}
\DeclareSIUnit\Mpc{\mega\pc}
\DeclareSIUnit\dex{dex}
\DeclareSIUnit\deg{deg}
\DeclareSIUnit\mag{mag}
\DeclareSIUnit\Jy{Jy}
\DeclareSIUnit\mJy{\milli\Jy}
\DeclareSIUnit\beam{beam}
\DeclareSIUnit\bvla{beam_{VLA}}
\DeclareSIUnit\bfast{beam_{FAST}}
\DeclareSIUnit\pixel{pixel}
\AtBeginDocument{\DeclareSIUnit[quantity-product={},list-units=repeat]\percent{\text{\%}}}

